MemOS: An Operating System for Memory-Augmented Generation (MAG) in Large Language Models

Large Language Models (LLMs) have emerged as foundational infrastructure in the pursuit of Artificial General Intelligence (AGI). Despite their remarkable capabilities in language perception and generation, current LLMs fundamentally lack a unified and structured architecture for handling memory. They primarily rely on parametric memory (knowledge encoded in model weights) and ephemeral activation memory (context-limited runtime states). While emerging methods like Retrieval-Augmented Generation (RAG) incorporate plaintext memory, they lack lifecycle management and multi-modal integration, limiting their capacity for long-term knowledge evolution. To address this, we introduce MemOS, a memory operating system designed for LLMs that, for the first time, elevates memory to a first-class operational resource. It builds unified mechanisms for representation, organization, and governance across three core memory types: parametric, activation, and plaintext. At its core is the MemCube, a standardized memory abstraction that enables tracking, fusion, and migration of heterogeneous memory, while offering structured, traceable access across tasks and contexts. MemOS establishes a memory-centric execution framework with strong controllability, adaptability, and evolvability. It fills a critical gap in current LLM infrastructure and lays the groundwork for continual adaptation, personalized intelligence, and cross-platform coordination in next-generation intelligent systems.

==> tab/osmapping.tex <==
\begin{table}[h]
\centering
\small
\caption{Mapping from Traditional OS to MemOS Components}
\label{table:mapping}
\begin{tabular}{p{3.0cm} p{3.0cm} p{3.5cm} p{5.5cm}}
\toprule
\textbf{Resource Type} & \textbf{OS Component} & \textbf{MemOS Component} & \textbf{Design Objective} \\
\midrule
\multicolumn{4}{c}{\textit{Process Management}} \\
\midrule
Core Execution & CPU Core & LLM Core & Inference and generation tasks \\
Scheduling & Scheduler & MemScheduler & Memory cube scheduling \\
Process Control & PCB & ITCB & Manage inference tasks and metadata \\
Context Switch & Context Switcher & Memory Context Switch & Switch active memory states \\
\midrule
\multicolumn{4}{c}{\textit{Memory Management}} \\
\midrule
Memory Layering & Virtual Memory & Memory Layering & Multi-level memory management \\
Page Table & Page Table & Memory Mapping & Map memory cube allocations \\
Swap Management & Swap Space & Frozen Memory Store & Offload inactive memories \\
Memory Cache & Cache System & Memory Cache & Fast memory access \\
\midrule
\multicolumn{4}{c}{\textit{Storage Management}} \\
\midrule
Persistent Storage & File System & MemVault & Manage multi-type memory vaults \\
System Calls & Syscall API & MemAPI & Standard memory APIs \\
I/O Handling & I/O Drivers & Backend Adapter & Storage backend abstraction \\
Package Deploy & Package Manager & MemStore & Publish and share memory bundles \\
\midrule
\multicolumn{4}{c}{\textit{Protection and Security}} \\
\midrule
Authentication & Auth Module & Memory Auth & Access verification for memories \\
ACL Management & ACLs & Memory ACL & Permission policies for memory cubes \\
Encryption & Encryption Module & Privacy Shield & Memory data protection \\
Logging & Syslog & Memory Log & Track memory operations \\
Anomaly Detection & Failure Detector & Hallucination Detector & Detect hallucination and faults \\
\bottomrule
\end{tabular}
\end{table}

==> tab/references.tex <==
\begin{table}[htbp]
\centering
\caption{记忆类型、运作机制与典型示例分类}
% \caption{Classification of Memory Types, Mechanisms, and Example References}
\label{tab:memory_classification}
\renewcommand{\arraystretch}{1.4}
\footnotesize
\begin{tabular}{m{0.08\textwidth} m{0.12\textwidth} m{0.23\textwidth} m{0.46\textwidth}}
\hline
\textbf{Timescale} & \textbf{Consciousness} & \textbf{Mechanism} & \textbf{Example References} \\ \hline

\multirow{4}{*}[-4ex]{\makecell[l]{Short-term}} 
& \multirow{1}{*}{\makecell[l]{Explicit}} 
& Prompt-Based Context 
& GPT-2 \cite{radford_gpt2_nodate}, GPT-3 \cite{brown_gpt3_2020}, Prefix-Tuning \cite{li_prefix-tuning_2021}, Prompt-Tuning \cite{lester_prompt-tuning_2021}, P-Tuning \cite{liu_ptuning_2023, liu_ptuningv2_2022}, InstructGPT \cite{ouyang_instructgpt_2022} \\ \cline{2-4}

& \multirow{3}{*}[-2ex]{\makecell[l]{Implicit}} 
& Key-Value Cache Mechanism 
& vLLM \cite{kwon_vLLM_2023}, StreamingLLM\cite{xiao_streamingllm_2023}, H2O\cite{zhang_h2o_2023}, LESS \cite{dong_less_2024}, KVQuant \cite{hooper_kvquant_2024}, RetrievalAttention \cite{liu_retrievalattention_2024}, Memory³ \cite{yang_memory3_2024} \\ \cline{3-4}

& 
& Hidden State Steering 
& Steer \cite{subramani_steerno1_2022}, ICV \cite{liu_ICV_2024}, ActAdd \cite{turner_ActAdd_2024}, StyleVec \cite{konen_stylevec_2024}, CAA \cite{rimsky_CAA_2024}, FreeCtrl \cite{feng_freectrl_2024}, EasyEdit2 \cite{xu_easyedit2_2025} \\ \cline{3-4}

& 
& Activation Circuit Modulation 
& SAC \cite{xiao_sac_2024}, DESTEIN \cite{li_destein_2024}, LM-Steer \cite{han_lmsteer_2024} \\ \hline

\multirow{4}{*}[-6ex]{\makecell[l]{Long-term}} 
& \multirow{1}{*}[-2ex]{\makecell[l]{Explicit}} 
&Non-parametric Retrieval-Augmented Generation 
& kNN-LMs \cite{khandelwal_knnlm_2019,pozzobon_goodtriever_2023},  MEMWALKER \cite{DBLP:journals/corr/abs-2310-05029}, Graph RAG \cite{DBLP:journals/corr/abs-2404-16130}, LightRAG \cite{DBLP:journals/corr/abs-2410-05779}, NodeRAG \cite{xu2025noderagstructuringgraphbasedrag,yang2025heteragheterogeneousretrievalaugmentedgeneration}, HyperGraphRAG \cite{DBLP:journals/corr/abs-2503-21322}, HippoRAG \cite{DBLP:conf/nips/GutierrezS0Y024,DBLP:journals/corr/abs-2502-14802}, PGRAG\cite{DBLP:journals/corr/abs-2405-16933}, Zep \cite{DBLP:journals/corr/abs-2501-13956}, A-MEM~\cite{DBLP:journals/corr/abs-2502-12110}, Mem0\cite{chhikara2025mem0buildingproductionreadyai} \\ \cline{2-4}



& \multirow{3}{*}[-4ex]{\makecell[l]{Implicit}} 
& Parametric Knowledge 
& BERT \cite{devlin_bert_2019}, RLHF \cite{bai_rlhf_2022}, CTRL \cite{keskar_ctrl_2019}, SLayer \cite{chen_slayer_2024} \\ \cline{3-4}

& 
& Modular Parameter Adaptation 
& LoRA \cite{hu_lora_2021}, PRAG \cite{su_PRAG_2025}, DyPRAG \cite{tan_DyPRAG_2025}, SERAC \cite{mitchell_serac_2022}, CaliNet \cite{dong_CaliNet_2022}, DPM \cite{cheng_DPM_2023}, GRACE \cite{hartvigsen_grace_2023} \\ \cline{3-4}

& 
& Parametric Memory Editing 
& ROME \cite{meng_rome_2023}, MEMIT \cite{meng_memit_2023}, AlphaEdit \cite{fang_alphaedit_2025}, AnyEdit \cite{jiang_anyedit_2025}, EasyEdit \cite{zhang_easyedit_2024}, AdaPLE \cite{li_AdaPLE_2024}, MEMAT \cite{tamayo_memat_2024} \\ \hline

\end{tabular}
\end{table}

